Performance of a Full-Size Small-Strip Thin Gap Chamber Prototype for the ATLAS New Small Wheel Muon Upgrade

The instantaneous luminosity of the Large Hadron Collider at CERN will be increased up to a factor of five with respect to the present design value by undergoing an extensive upgrade program over the coming decade. The most important upgrade project for the ATLAS Muon System is the replacement of the present first station in the forward regions with the so-called New Small Wheels (NSWs). The NSWs will be installed during the LHC long shutdown in 2018/19. Small-Strip Thin Gap Chamber (sTGC) detectors are designed to provide fast trigger and high precision muon tracking under the high luminosity LHC conditions. To validate the design, a full-size prototype sTGC detector of approximately 1.2 $\times$ $1.0\, \mathrm{m}^2$ consisting of four gaps has been constructed. Each gap provides pad, strip and wire readouts. The sTGC intrinsic spatial resolution has been measured in a $32\, \mathrm{GeV}$ pion beam test at Fermilab. At perpendicular incidence angle, single gap position resolutions of about $50\,\mathrm{\mu m}$ have been obtained, uniform along the sTGC strip and perpendicular wire directions, well within design requirements. Pad readout measurements have been performed in a $130\, \mathrm{GeV}$ muon beam test at CERN. The transition region between readout pads has been found to be $4\,\mathrm{mm}$, and the pads have been found to be fully efficient.

==> tex/fermilab_calibration.tex <==
text, figures
